Super Mario in the Pernicious Kingdoms: Classifying glitches in old games

In a case study spanning four classic Super Mario games and the analysis of 237 known glitches within them, we classify a variety of weaknesses that are exploited by speedrunners to enable them to beat games quickly and in surprising ways. Using the Seven Pernicious Kingdoms software defect taxonomy and the Common Weakness Enumeration, we categorize the glitches by the weaknesses that enable them. We identify 7 new weaknesses that appear specific to games and which are not covered by current software weakness taxonomies.

==> data/out/glitch-counts.tex <==
\begin{tabular}{lrr}
  \toprule
  Game & Glitches & Mappings \\
  \midrule
  \acl{SMB1} & 32 & 16 \\
  \acl{SMB3} & 54 & 19 \\
  \acl{SMW} & 36 & 17 \\
  \acl{SM64} & 115 & 19 \\
  \midrule
  Total & 237 & 32 \\
  \bottomrule
\end{tabular}

